Predicting vs. Acting: A Trade-off Between World Modeling & Agent Modeling

RLHF-aligned LMs have shown unprecedented ability on both benchmarks and long-form text generation, yet they struggle with one foundational task: next-token prediction. As RLHF models become agent models aimed at interacting with humans, they seem to lose their world modeling -- the ability to predict what comes next in arbitrary documents, which is the foundational training objective of the Base LMs that RLHF adapts. Besides empirically demonstrating this trade-off, we propose a potential explanation: to perform coherent long-form generation, RLHF models restrict randomness via implicit blueprints. In particular, RLHF models concentrate probability on sets of anchor spans that co-occur across multiple generations for the same prompt, serving as textual scaffolding but also limiting a model's ability to generate documents that do not include these spans. We study this trade-off on the most effective current agent models, those aligned with RLHF, while exploring why this may remain a fundamental trade-off between models that act and those that predict, even as alignment techniques improve.

==> fig/fig-freq-sharing.tex <==
\begin{figure}
\centering \footnotesize

\includegraphics[width=1\linewidth]{img/freq_sharing.png}

\caption{
\textbf{frequency of character sharing}
}
\label{fig:freq-sharing}
\end{figure}

==> fig/fig-non-neg.tex <==
\begin{figure*}[!ht]
\centering \footnotesize
% 

\begin{minipage}{0.45\textwidth}
 \centering
 \includegraphics[width=1\linewidth]{img/non-negligible_7b_style.png}
 \textbf{(A)}
\end{minipage}
\begin {minipage}{0.45\textwidth}
 \centering
 \includegraphics[width=1\linewidth]{img/non-negligible_70b_style.png}
 \textbf{(B)}
\end{minipage}

\caption{
\textbf{(\S\ref{sec:collapse}) RLHF models assign near-zero probability mass to almost all tokens when generating, more than Base models.} For both \textbf{(A)} 7B and \textbf{(B)} 70B models, RLHF models assign non-negligible ($> 1E-8$) probability to \emph{significantly fewer} vocabulary tokens when predicting next tokens from its own generations (nucleus sampling, p = 0.9), but slightly \emph{more} tokens when predicting next tokens on gold text sequences. This suggests collapse for RLHF models only in their generative distributions. Details are in Appendix \ref{sec:setup-topk}.
}
\label{fig:non-neg}
\end{figure*}

==> fig/fig-probing-old.tex <==
\begin{figure}[t]
\centering \footnotesize

\begin{minipage}{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{img/linear_probing_pile_small.png}
    \textbf{(A)}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{img/linear_probing_pile_other_small.png}
    \textbf{(B)}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{img/linear_probing_anthropic_small.png}
    \textbf{(C)}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{img/linear_probing_anthropic_other_small.png}
    \textbf{(D)}
\end{minipage}
\caption{
\textbf{
(\S\ref{sec:predict_future}) The intermediate representations of RLHF models contain more easily extracted information (by a linear probe) for predicting their own future tokens, compared to Base models.}  We train a linear model to predict each model's future tokens ($n=1,2,3$ tokens into the future) given the hidden representation. \textbf{(A)} Linear probe accuracy, given a model's hidden representation, on prediction of a token $n$ steps into the future of the same model's generation, conditioned on a short prompt from the Pile. \textbf{(B)} Similar to (A), but predicting tokens in the future of the other (Base for RLHF, and vice versa) model's generation. \textbf{(C)} Similar to (A), but predicting future tokens in the model's own generations, conditioned on prompts from the Anthropic Helpful dataset. \textbf{(D)} Similar to (C), but predicting tokens in the future of the other model's generation.}
\label{fig:probing}
\end{figure}

==> sections/backups/1_introduction_v0.tex <==
\input{fig/fig-1}

\section{Introduction}
\label{sec:intro}
 {}

Alignment with RLHF \citep{ivison2023camels,touvron2023llama} pushes models towards action: completing specific goals and excelling across both short and long-form textual tasks. RLHF adapts base LMs that are trained to be \emph{world models}, accurately predicting the distribution of text that might occur after an arbitrary prefix. Base LMs have complex abilities such as simulating documents from the internet, and while RLHF models tend to excel at complex tasks, in this work we find that they seem to have lost these \emph{world modeling} abilities. We propose that this trade-off is a natural result of RLHF models concentrating probability to specific spans, which allows these models to blueprint long-form generation (Figure~\ref{fig:fig1}) but reduces their ability to model arbitrary text. %\peter{Needs a bit of work + shortening, but I tried to incorporate justification for why we even care about world modeling (i.e. why we don't just see it as ``priming'' but an actually useful task)}

Specifically, RLHF models struggle with next-token prediction which directly measures ability to world model, even when they are finetuned to regain these skills (\S\ref{sec:notllms}). RLHF models seem to concentrate probability on a smaller set of text (\S\ref{sec:collapse}), related to distributional collapse from past work \citep{shumailov2023curse}. Yet this concentration may have a use, in making generation more self-predictable, and helping to blueprint long-form text generations. For example, we find \emph{anchor spans} (Figure~\ref{fig:fig1}) which appear across many samples for the same prompt, and seem to serve as scaffolding for generation (\S\ref{sec:planning}).

Is this trade-off between world modeling and agent modeling fundamental? Intuitively, agent models may need to concentrate probability and information to \emph{act} which would be at odds with the openness to all possibilities needed to \emph{predict}--we see this at least with these RLHF-adapted agents. 

%RLHF alignment \citep{ivison2023camels,touvron2023llama} pushes language models--trained to capture the probability of arbitrary text--to complete goals and take specific action. Yet, while we find that RLHF makes models better at \emph{agent modeling}, they seem to lose \emph{world modeling}, or the ability to predict the probability of arbitrary text that the base LMs excel at. In this work, we propose that this trade-off is a natural result of RLHF models concentrating probability to specific spans, which allows these models to blueprint long-form generation while reducing their ability to model arbitrary text. 

% Alignment with RLHF \citep{ivison2023camels,touvron2023llama} pushes models towards action--completing specific goals--and builds on language that try to capture the overall distribution of text. Yet, these two objectives seem to be at odds--while we find that RLHF models get better at \emph{agent modeling}, they seem to lose \emph{world modeling}, or the ability to predict the probability of arbitrary text that the base LMs excel at. 


%Alignment with RLHF \citep{ivison2023camels,touvron2023llama} has been a key ingredient in recent language model development, pushing towards \emph{\agents} which complete goals with impressive effectiveness in long-form text generation.

%Large language models (LLMs), trained as next-token-predictors, must be \textit{reactive}: predictions made immediately after a surprising token must adjust and reinterpret previous context. This reactivity allows models to act like a diverse set of authors with myriad possible goals \citep{andreas-2022-language}, but is also a significant factor in why large language models are easily derailed by even a single token.



%When a human writes an essay, they usually have an idea in mind, and route themselves back to the original plan if they find themselves falling off track. This is the behavior expected of \textit{agent models} that attempt to complete long-term goals over many timesteps. We show that LLMs which have been adapted to \agenting{} through Reinforcement Learning from Human Feedback \citep{ouyang2022training} implicitly contain blueprints for long-form generation, which arise by concentrating the distribution of possible future text into a limited set of options.



%Is there a trade-off between reactive \worldmodeling{} and \agenting{} that involves long-form planning? Intuitively, this seems plausible. World modeling involves guessing a mixture of different possible authors and contexts to sample from, while \agenting{} attempts to represent a more-or-less singular speaker completing goals that are further out than one-token in the future. 

As we show in this paper, agent-adapted language models are no longer as effective at base language modeling—even when finetuned to become base language models again. %\peter{Either here or earlier, want to drive home that this is a kind of general knowledge of language that they lose, not just some specific task} \peter{After reading the whole thing again, pushing even harder on this. A lot of people won't see why being a good LM is important at all, other than implicitly} 
While there are likely multiple factors causing this diminished performance, a key aspect is \textit{distribution collapse }~\citep{shumailov2023curse}, or \emph{concentration of probability}. Agent models are less diverse on multiple axes. They produce fewer unique \textit{n}grams for the same prompt, assign higher probability to their own sampled generations, and assign near-zero probability to significantly more tokens in the vocabulary. \peter{Reads a bit negative}



This collapse\peter{concentration?} is not uniform. We show that current \agents{} have an implicit blueprint of ``\nervecenterspans{}'': spans of text shared across different generations sampled from the same prompt, which the model tends to keep in approximately the same order; see Figure~\ref{fig:fig1} for an initial example. In essence, current models trained with RLHF tend to have an implicit list of points to hit when given a prompt, something that even base language models with similarly low diversity (achieved using a lower $p$ in nucleus sampling) do not have.

We posit that this distribution shrinkage\peter{concentration?} \ari{shrinkage is cute, but we can't have collapse, shrinkage, and concentration, we need more uniformity} \peter{My feeling is, we stick with collapse (as the legible one) and concentraion (as our introduced term)} is likely an inevitable aspect of \agents{}, not just a spurious byproduct of RLHF. In order to generate coherent long-form responses (or act towards goals in general) an agent must guarantee that its future actions are largely predictable to its current self. \peter{This is a great explanation of ``predictability''--perhaps push it throughout to other mentions of this} In effect, \emph{agent modeling} may require minimizing long-term uncertainty while \emph{world modeling} requires maintaining the true uncertainty of natural text documents, a fundamental trade-off. \ari{let's get the intro all on one page, then include an image of it in the final tweet}

%Language models cannot minimize long-term uncertainty and still perform well at \prediction{}, since they are designed to react to new context, model any possible document, disregarding their own future generations in the prediction process. \peter{Simplify this sentence to make it instantly click--something like depth vs breadth or being open vs deliberate. Not sure.}

==> sections/backups/plan_v0.tex <==
\section{Agent models think ahead}
\label{sec:planning}

\input{fig/fig-probing}

We have shown that RLHF models are no longer good \predictors{} and that they collapse their probability distributions into more predictable outcomes. What does this probabilty mass shift lead to? In this section we show evidence that RLHF models make use of a kind of implicit blueprints for long-form generation rather than predicting only one token in advance, effectively using concentrated probability to enable ``thinking ahead'' in long form generation. \peter{Connect this slightly more to section title?} \peter{Tried, may be too inexact. Check it}

\subsection{RLHF hidden states are more predictive of future tokens}
\label{sec:predict_future}

%\peter{``We first test how much information models have about their future actions, beyond the next step'' or something} 
As a basic measure of ``thinking ahead'', we estimate the information models have about future timesteps, beyond the next token. Using the methodology of \citet{pal2023future}, we study how well we can predict tokens for Llama 2 7B Base and RLHF models by leveraging their own hidden states.
Specifically, we perform evaluation on the Pile~\citep{gao2020pile} and Anthropic Helpful~\citep{bai2022training} datasets.
We train a linear model on the hidden representation from the 28th layer (Llama 2 7B comprises 32 layers), using 100,000 tokens from each dataset, to predict tokens $n$ steps into the future ($n=1, 2, 3$), \textit{after} the token being predicted at the current timestep. We use this prediction accuracy as a metric to assess the effectiveness of using a model's hidden state to foresee its own generation of future tokens.

% For evaluation, we measure the accuracy, indicating how well we can predict the future generated tokens of the Base and RLHF models only using their own hidden states. 


Linear probes on RLHF models can predict future tokens in their own generations with higher accuracy than Base models (Figure~\ref{fig:probing}). RLHF adapted models find it easier to predict the future because they generate a future that is more predictable, as supported by Figure~\ref{fig:self-perplexity-llama}.
%In \S\ref{sec:tradeoff} we argue that this will be an inherent feature of density functions that are optimized for use as \agents{}. \swj{not too sure about the density function}

Figure~\ref{fig:probing} also shows that RLHF models may contain a subset of information that base LLMs do, as base LLMs are more effective at predicting future tokens of RLHF models than the reverse. This supports the idea of concentration or collapse in RLHF models, as their predictions fit base LLMs, but they no longer explain base LLM predictions as effectively. \peter{Maybe transition to next}


%Figure~\ref{fig:probing} also shows us that the predictable distribution RLHF models occupy is likely a subdistribution of the Base LLM they were adapted from. Specifically, base LLMs contain more predictive information about future tokens of RLHF models than the reverse. 

%\peter{Subdistribution is a little too simple because we're training probes. Not directly subdistr}

%Specifically, Base LLMs are better at predicting future tokens for RLHF models than the reverse. This asymmetry suggests that RLHF models are not simply shifting in distribution, they are occupying a less expressive subset of the original, that is well captured by the base LLMs. % Since the Base model can more reliably predict the RLHF-adapted model than the reverse, it is likely that relevant features from the original model are collapsed and no longer recoverable from the RLHF-adapted model. 
%\peter{This can be a lot shorter/clearer I think. (redundancy)} %\peter{Point is made well here but probably needs to be hedged/softened}


\subsection{Sampled generations contain align-able backbones}
\label{sec:backbones}

\input{fig/fig-ngrams}

\peter{I would think about flipping order of this and the next section maybe? I think it will be easier to lead with the intuitive examples, and then support it with the quantitative results (same as the strategy in fig 1). Although I see the appeal of this way, begin with numerical findings and propose a hypothesis. But I think the issue here is that the hypothesis, being surface forms, feels also like an observation. Thinking about it}
RLHF models seem to construct implicit blueprints for a given prompt, consistently touching on certain points across different samples. Sampling 100 continuations for the same prompt from an RLHF model leads to sequences with a significant amount of diversity (in terms of unique $n$grams), but a surprisingly high amount of overlap between the sequences. Initially, these two statements may appear to be in conflict, but Figure~\ref{fig:ngrams} shows this is not the case. We can use nucleus sampling \citep{holtzman2020curious} to generate text with similar $n$gram diversity across Base LLMs and RLHF-adapted models by setting the value of $p$ appropriately (see Appendix \ref{sec:planning-experiments}). Yet even when diversity statistics are similar, RLHF models reuse more long $n$grams across different generations for the same prompt than models not trained using Reinforcement Learning.
In Figure~\ref{fig:ngrams}, on average a quarter of RLHF outputs share at least one 25-gram (about a sentence), and there are almost twice as many RLHF sequences sharing at least a 10-gram than for the Base model. This high level of \textit{n}gram sharing is not limited to a few isolated cases or to the prefix or suffix of the generations. The bar-chart on the right side of Figure~\ref{fig:ngrams}~(B) shows that on average 10-grams are shared by more sequences in RLHF model outputs by a large margin (note log-scale).

However, \textit{n}gram statistics are not robust to small variations, nor do they consider ordering effects—where \textit{n}grams in RLHF models tend to occur in certain orders. 
To handle these problems, we propose to first align the continuations for a given prompt sequence alignment software originally developed for bioinformatics, MAFFT \citep{katoh2013mafft}.
% originally first using off-the-shelf

After aligning 100 continuations for each prompt (Figure~\ref{fig:fig1}, bottom), Base models have a much lower overlap compared to RLHF models despite having controlled for \textit{n}gram diversity using the nucleus sampling parameter $p$, as described in Appendix~\ref{sec:planning-experiments}. RLHF models have significantly more overlap for all positions, and at the beginning and end of the sequences the overlap is even more drastic. This shows that RLHF models tend to converge back towards the end of the generations. Additionally, we note that the larger confidence intervals (shaded in the figure) indicate that the convergence points occur at different positions in the sequences for different prompts. These results hold true across different models, see Appendix~\ref{app:overlap}.

\input{fig/fig-sankey}


\subsection{Anchor spans as an implicit blueprint}
\label{sec:anchor_spans}

If RLHF models blueprint long-form texts out in advance, what do these blueprints look like? To characterize the overlapping sequences implied by Figure~\ref{fig:fig1} (bottom), we visualize the alignments with Sankey diagrams Figure~\ref{fig:fig1}~(top), which characterize the flow through critical nodes over a sequential process. We focus on  ``anchor spans''—substrings that occur across many sampled outputs for the same prompt—such that the flow between two nodes $A$ and $B$ represents the set of generations which contain $A$, followed by $B$, with (possibly different) text in between. Specifically, we first identify all text spans of a fixed minimum length (30 characters), which occur at a specific index for at least some threshold number of generations (20\%). If the same span occurs at two different positions in the alignment indexing, they are counted as different spans. We sort the spans in descending order of frequency across unique outputs, and then by span length. We then greedily pick up to a maximum (6 in these visualizations) number of spans, updating the occurrence counts for unpicked spans after each addition, so that generations cannot ``double count'' for spans which overlap. See Appendix \ref{sec:planning-experiments} for further details.


RLHF models blueprint their long-form generations: Figure~\ref{fig:sankey}~(top) shows that anchor spans remain constant across many outputs, analogous to a bullet point outline embedded within a generation. Figure~\ref{fig:sankey}~(bottom) shows that for the same prompt the Base model (Llama 2 70B) has no such structure whatsoever, even when using a more restricted sampling strategy. In other words, %\peter{Maybe rather than ``plan'' we can use a word people must admit is true, like ``many elements of content seem to be predetermined''. Not this but something clearer} \ari{try this on} 
RLHF models rely on an implicit blueprint, converging to certain spans from which they can reliably predict their own future, while Base models diverge in unpredictable ways (more examples Appendix~\ref{sec:appendix-sankey}).

==> sections/backups/plan_v1.tex <==
\section{Agent models think ahead}
\label{sec:planning}

\input{fig/fig-probing}

We have shown that RLHF models are no longer good \predictors{} and that they concentrate their probability distributions into more predictable outcomes. What does this probability mass shift lead to? In this section we show evidence that RLHF models make use of a kind of implicit blueprint for long-form generation rather than predicting only one token in advance, effectively using probability concentrated on certain future spans to enable ``thinking ahead'' in long form generation. 

\subsection{RLHF hidden states are more predictive of future tokens}
\label{sec:predict_future}

%\peter{``We first test how much information models have about their future actions, beyond the next step'' or something} 
As a basic measure of ``thinking ahead'', we estimate the information models have about future timesteps, beyond the next token. Using the methodology of \citet{pal2023future}, we study how well we can predict tokens for Llama 2 7B Base and RLHF models by leveraging their own hidden states and a linear probe.
Specifically, we perform evaluation on the Pile~\citep{gao2020pile} and Anthropic Helpful~\citep{bai2022training} datasets.
We train a linear model on the hidden representation from the 28th layer (Llama 2 7B comprises 32 layers), using 100,000 tokens from each dataset, to predict tokens $n$ steps into the future ($n=1, 2, 3$), \textit{after} the token being predicted at the current timestep. We use this prediction accuracy as a metric to assess the effectiveness of using a model's hidden state to foresee its own generation of future tokens.

% For evaluation, we measure the accuracy, indicating how well we can predict the future generated tokens of the Base and RLHF models only using their own hidden states. 


Linear probes on RLHF models can predict future tokens in their own generations with higher accuracy than Base models (Figure~\ref{fig:probing}). RLHF adapted models find it easier to predict the future because they generate a future that is more predictable, as supported by Figure~\ref{fig:self-perplexity-llama}.
%In \S\ref{sec:tradeoff} we argue that this will be an inherent feature of density functions that are optimized for use as \agents{}. \swj{not too sure about the density function}

Figure~\ref{fig:probing} also shows that RLHF models may contain a subset of information that base LLMs do, as base LLMs are more effective at predicting future tokens of RLHF models than the reverse. This supports the idea of concentration or collapse in RLHF models, as their predictions fit base LLMs, but they no longer explain base LLM predictions as effectively. 


%Figure~\ref{fig:probing} also shows us that the predictable distribution RLHF models occupy is likely a subdistribution of the Base LLM they were adapted from. Specifically, base LLMs contain more predictive information about future tokens of RLHF models than the reverse. 

%\peter{Subdistribution is a little too simple because we're training probes. Not directly subdistr}

%Specifically, Base LLMs are better at predicting future tokens for RLHF models than the reverse. This asymmetry suggests that RLHF models are not simply shifting in distribution, they are occupying a less expressive subset of the original, that is well captured by the base LLMs. % Since the Base model can more reliably predict the RLHF-adapted model than the reverse, it is likely that relevant features from the original model are collapsed and no longer recoverable from the RLHF-adapted model. 
%\peter{This can be a lot shorter/clearer I think. (redundancy)} %\peter{Point is made well here but probably needs to be hedged/softened}


\subsection{Anchor spans as an implicit blueprint}
\label{sec:anchor_spans}

Besides containing more information about next tokens, RLHF models seem to qualitatively \emph{blueprint} generations, consistently using the same key points across many generations for a given prompt (Figure~\ref{fig:fig1}~top). Base LLMs show no such structure (Figure~\ref{fig:sankey}~bottom).

We visualize these blueprints with Sankey diagrams (Figure~\ref{fig:fig1}~top), which characterize the flow through critical nodes over a sequential process. We focus on  ``anchor spans''—substrings that occur across many sampled outputs for the same prompt—such that the flow between two nodes $A$ and $B$ represents the set of generations which contain $A$, followed by $B$, with (possibly different) text in between. Specifically, we first identify all text spans of a fixed minimum length (30 characters), which occur at a specific index for at least some threshold number of generations (20\%). If the same span occurs at two different positions in the alignment indexing, they are counted as different spans. We sort the spans in descending order of frequency across unique outputs, and then by span length. We then greedily pick up to a maximum (6 in these visualizations) number of spans, updating the occurrence counts for unpicked spans after each addition, so that generations cannot ``double count'' for spans which overlap. See Appendix \ref{sec:planning-experiments} for further details.


Qualitatively, RLHF models seem to blueprint their long-form generations: Figure~\ref{fig:sankey}~(top) shows that anchor spans remain constant across many outputs, analogous to a bullet point outline embedded within a generation.  For the same prompt the Base model (Llama 2 70B) has no such structure whatsoever, even when using a more restricted sampling strategy (Figure~\ref{fig:sankey}~bottom). In other words, %\peter{Maybe rather than ``plan'' we can use a word people must admit is true, like ``many elements of content seem to be predetermined''. Not this but something clearer} \ari{try this on} 
RLHF models rely on an implicit blueprint, converging to certain spans from which they can reliably predict their own future, while Base models diverge in unpredictable ways (more examples Appendix~\ref{sec:appendix-sankey}).


\subsection{Sampled generations contain align-able backbones}
\label{sec:backbones}

\input{fig/fig-ngrams}

%\peter{!!! could make this intro a bit better}

The blueprints in \S\ref{sec:anchor_spans} appear quantitatively as well, as the degree of alignment possible across multiple generations. Sampling 100 continuations for the same prompt from an RLHF model leads to sequences with a significant amount of diversity (in terms of unique $n$grams), but a surprisingly high amount of overlap between the sequences. While diversity and overlap may seem to be in conflict, Figure~\ref{fig:ngrams} shows this is not the case. We can use nucleus sampling \citep{holtzman2020curious} to generate text with similar $n$gram diversity across Base LLMs and RLHF-adapted models by setting the value of $p$ appropriately (see Appendix \ref{sec:planning-experiments}). Yet even when diversity statistics are similar, RLHF models reuse more long $n$grams across different generations for the same prompt than models not trained using Reinforcement Learning. In effect, the diversity is not evenly distributed in RLHF generation, with diversity concentrated in between predictable, long spans.

In Figure~\ref{fig:ngrams}, on average a quarter of RLHF outputs share at least one 25-gram (about a sentence), and there are almost twice as many RLHF sequences sharing at least a 10-gram than for the Base model. This high level of \textit{n}gram sharing is not limited to a few isolated cases or to the prefix or suffix of the generations. The bar-chart on the right side of Figure~\ref{fig:ngrams}~(B) shows that on average 10-grams are shared by more sequences in RLHF model outputs by a large margin (note log-scale).

However, \textit{n}gram statistics are not robust to small variations, nor do they consider ordering effects—where \textit{n}grams in RLHF models tend to occur in certain orders. 
To handle these problems, we propose to first align the continuations for a given prompt sequence alignment software originally developed for bioinformatics, MAFFT \citep{katoh2013mafft}.
% originally first using off-the-shelf

After aligning 100 continuations for each prompt (Figure~\ref{fig:fig1}, bottom), Base models have a much lower overlap compared to RLHF models despite having controlled for \textit{n}gram diversity using the nucleus sampling parameter $p$, as described in Appendix~\ref{sec:planning-experiments}. RLHF models have significantly more overlap for all positions, and at the beginning and end of the sequences the overlap is even more drastic. This shows that RLHF models tend to converge back towards the end of the generations. Additionally, we note that the larger confidence intervals (shaded in the figure) indicate that the convergence points occur at different positions in the sequences for different prompts. These results hold true across different models, see Appendix~\ref{app:overlap}.

\input{fig/fig-sankey}



